Reinforcement Learning from Real-Robot Interaction without High-Quality State Estimates

A longstanding goal for robot reinforcement learning (RL) is that robots learn from their own physical experience, as humans and animals do. A key obstacle to learning directly from physical experience, especially outside instrumented lab environments, is that the state of the world is usually unobservable to the learner and must be estimated from on-board sensing. Errors in that estimate corrupt both the policy input and potentially the reward signal. We study this challenge using the contact-rich task of a bipedal robot learning to score soccer goals. We estimate all key state variables on-board with an unscented Kalman filter (UKF) and no external instrumentation (e.g., motion capture or overhead cameras). Because the UKF may incorrectly estimate state when the ball is unobserved, we learn a new state representation with a recurrent state-space model (RSSM) that, critically, only corrects the RSSM's latent state when the ball is observed. Building on RLPD, we introduce RSSM-RLPD and apply it to the task of a NAO robot learning to dribble a soccer ball into a goal. We show that the robot learns to score from multiple starting positions after 30 minutes of real-world interaction, reaching 100% success against 0% for a feed-forward policy under the same training budget. We complement our physical robot experiments with a simulation study and show that RSSM-RLPD learns policies that achieve a higher success rate than behavior cloning, a feed-forward, and GRU baseline. Taken together, our results show that the addition of a learned state representation to existing on-robot learning methods enables RL from real-robot data even with a high degree of partial observability.

==> figures/conditions_inline.tex <==
\begin{figure*}[t]
\centering
\definecolor{paperrssmrlpd}{HTML}{b12935}
\definecolor{papergrurlpd}{HTML}{1769a4}
\definecolor{paperffrlpd}{HTML}{d88700}
\definecolor{paperbc}{HTML}{646b73}
\begin{tikzpicture}
\begin{groupplot}[group style={group size=3 by 1,horizontal sep=0.45cm},
width=0.27\textwidth,height=4.8cm,scale only axis,
xmin=-15,xmax=30,ymin=-0.6,ymax=6.6,y dir=reverse,
ytick={0,1,2,3,4,5,6},xtick distance=10,xlabel={Success difference (pp)},
axis lines*=left,xmajorgrids,grid style={gray!20},
label style={font=\footnotesize},tick label style={font=\scriptsize},title style={font=\footnotesize}]
\nextgroupplot[title={RSSM--RLPD minus GRU-RLPD},yticklabels={Nominal,Static blackout,Visible kick,Moving-ball loss,Occluder,Hidden kick,Overall}]
\addplot[gray,thin,forget plot] coordinates {(0,-0.6) (0,6.6)};
\addplot[only marks,mark=*,mark size=1.4pt,papergrurlpd,error bars/.cd,x dir=both,x explicit] table[x=x,y=y,x error minus=lo,x error plus=hi,row sep=\\] {
x y lo hi\\
2.91666667 0 9.58333333 9.16666667\\
0.41666667 1 8.75000000 9.16666667\\
3.33333333 2 6.66666667 7.08333333\\
-1.66666667 3 8.75000000 8.75000000\\
0.41666667 4 11.66666667 11.25000000\\
2.08333333 5 6.25000000 7.50000000\\
1.25000000 6 3.75000000 3.54166667\\
};
\nextgroupplot[title={RSSM--RLPD minus FF-RLPD},yticklabels={,,,,,,}]
\addplot[gray,thin,forget plot] coordinates {(0,-0.6) (0,6.6)};
\addplot[only marks,mark=*,mark size=1.4pt,paperffrlpd,error bars/.cd,x dir=both,x explicit] table[x=x,y=y,x error minus=lo,x error plus=hi,row sep=\\] {
x y lo hi\\
16.66666667 0 7.91666667 8.75000000\\
9.16666667 1 6.25000000 7.50000000\\
8.75000000 2 6.25000000 7.50000000\\
12.91666667 3 6.66666667 7.50000000\\
16.66666667 4 7.50000000 8.75000000\\
5.41666667 5 4.58333333 6.25000000\\
11.59722222 6 3.88888889 4.37673611\\
};
\nextgroupplot[title={RSSM--RLPD minus BC},yticklabels={,,,,,,}]
\addplot[gray,thin,forget plot] coordinates {(0,-0.6) (0,6.6)};
\addplot[only marks,mark=*,mark size=1.4pt,paperbc,error bars/.cd,x dir=both,x explicit] table[x=x,y=y,x error minus=lo,x error plus=hi,row sep=\\] {
x y lo hi\\
4.58333333 0 8.33333333 8.33333333\\
8.75000000 1 6.66666667 7.91666667\\
8.75000000 2 6.25000000 7.50000000\\
12.91666667 3 6.66666667 7.50000000\\
8.33333333 4 9.16666667 9.16666667\\
5.00000000 5 4.16666667 6.25000000\\
8.05555556 6 3.81944444 4.09722222\\
};
\end{groupplot}
\end{tikzpicture}
\caption{Held-out goal-success differences scored by simulator ground-truth goal crossing at the fixed 100k checkpoint (BC: zero online transitions), with 240 paired episodes per method and condition. Points and bars show means and 95\% hierarchical bootstrap intervals. All conditions share the same bootstrap draws. The solid vertical line marks zero.}
\label{fig:sealed_conditions}
\end{figure*}


==> figures/learning_curve_inline.tex <==
\begin{figure}[h]
\centering
\definecolor{paperrssmrlpd}{HTML}{b12935}
\definecolor{papergrurlpd}{HTML}{1769a4}
\definecolor{paperffrlpd}{HTML}{d88700}
\definecolor{paperbc}{HTML}{646b73}
\begin{tikzpicture}
\begin{axis}[
width=\columnwidth,height=4.65cm,scale only axis=false,
xmin=0,xmax=100,ymin=0,xtick={0,20,40,60,80,100},
xlabel={Online transitions (thousands)},ylabel={Goal success (\%)},
label style={font=\footnotesize},tick label style={font=\scriptsize},
axis lines*=left,ymajorgrids,grid style={gray!20},
legend style={font=\scriptsize,draw=none,at={(0.5,1.05)},anchor=south,legend columns=2,/tikz/every even column/.append style={column sep=3pt}},
legend cell align={left}]
\addplot[name path=paperrssmrlpdlow,draw=none,forget plot] coordinates {(0,0.00000000) (10,0.00000000) (20,1.66666667) (30,4.37500000) (40,3.33333333) (50,5.83333333) (60,2.91666667) (80,4.16666667) (100,1.66666667)};
\addplot[name path=paperrssmrlpdhigh,draw=none,forget plot] coordinates {(0,0.00000000) (10,3.75000000) (20,11.45833333) (30,18.75000000) (40,16.25000000) (50,16.66666667) (60,13.12500000) (80,15.62500000) (100,10.41666667)};
\addplot[paperrssmrlpd,fill opacity=0.08,draw=none,forget plot] fill between[of=paperrssmrlpdlow and paperrssmrlpdhigh];
\addplot[paperrssmrlpd,line width=0.85pt,mark=*,mark size=1.05pt] coordinates {(0,0.00000000) (10,1.25000000) (20,5.41666667) (30,10.83333333) (40,8.95833333) (50,10.83333333) (60,7.29166667) (80,9.16666667) (100,5.41666667)};
\addlegendentry{\method{}}
\addplot[name path=papergrurlpdlow,draw=none,forget plot] coordinates {(0,0.00000000) (10,2.08333333) (20,2.50000000) (30,0.83333333) (40,1.45833333) (50,1.25000000) (60,1.87500000) (80,1.87500000) (100,5.20833333)};
\addplot[name path=papergrurlpdhigh,draw=none,forget plot] coordinates {(0,0.00000000) (10,10.62500000) (20,11.66666667) (30,8.33333333) (40,7.91666667) (50,12.08333333) (60,12.29166667) (80,15.41666667) (100,17.29166667)};
\addplot[papergrurlpd,fill opacity=0.08,draw=none,forget plot] fill between[of=papergrurlpdlow and papergrurlpdhigh];
\addplot[papergrurlpd,line width=0.85pt,mark=*,mark size=1.05pt] coordinates {(0,0.00000000) (10,6.04166667) (20,6.45833333) (30,3.95833333) (40,4.37500000) (50,5.62500000) (60,6.45833333) (80,7.50000000) (100,10.41666667)};
\addlegendentry{\grumethod{}}
\addplot[name path=paperffrlpdlow,draw=none,forget plot] coordinates {(0,0.00000000) (10,0.00000000) (20,0.00000000) (30,0.00000000) (40,0.00000000) (50,0.00000000) (60,0.00000000) (80,0.00000000) (100,0.00000000)};
\addplot[name path=paperffrlpdhigh,draw=none,forget plot] coordinates {(0,0.00000000) (10,0.00000000) (20,0.00000000) (30,0.00000000) (40,0.00000000) (50,0.00000000) (60,0.00000000) (80,0.00000000) (100,3.33333333)};
\addplot[paperffrlpd,fill opacity=0.08,draw=none,forget plot] fill between[of=paperffrlpdlow and paperffrlpdhigh];
\addplot[paperffrlpd,line width=0.85pt,mark=*,mark size=1.05pt] coordinates {(0,0.00000000) (10,0.00000000) (20,0.00000000) (30,0.00000000) (40,0.00000000) (50,0.00000000) (60,0.00000000) (80,0.00000000) (100,0.83333333)};
\addlegendentry{FF-RLPD}
\addplot[name path=paperbclow,draw=none,forget plot] coordinates {(0,0.20833333) (10,0.20833333) (20,0.20833333) (30,0.20833333) (40,0.20833333) (50,0.20833333) (60,0.20833333) (80,0.20833333) (100,0.20833333)};
\addplot[name path=paperbchigh,draw=none,forget plot] coordinates {(0,3.54166667) (10,3.54166667) (20,3.54166667) (30,3.54166667) (40,3.54166667) (50,3.54166667) (60,3.54166667) (80,3.54166667) (100,3.54166667)};
\addplot[paperbc,fill opacity=0.08,draw=none,forget plot] fill between[of=paperbclow and paperbchigh];
\addplot[paperbc,line width=0.85pt,dashed,mark=none] coordinates {(0,1.66666667) (10,1.66666667) (20,1.66666667) (30,1.66666667) (40,1.66666667) (50,1.66666667) (60,1.66666667) (80,1.66666667) (100,1.66666667)};
\addlegendentry{BC (offline)}
\end{axis}
\end{tikzpicture}
\caption{Validation learning curves scored by simulator ground-truth goal crossing, over five training seeds with 480 paired episodes per method and checkpoint. Bands are pointwise 95\% hierarchical bootstrap intervals. BC is a single offline evaluation reused as a horizontal reference.}
\label{fig:validation_learning}
\end{figure}


==> figures/method_overview_inline.tex <==
% Standalone inline figure. Requires TikZ with arrows.meta and positioning.
% Maximum diagram width is 8.2 cm; no external graphics are required.
\begin{figure}[h]
\centering
\begin{tikzpicture}[
    x=1cm,y=1cm,
    font=\scriptsize,
    block/.style={draw=black!65,rounded corners=2pt,align=center,
        inner sep=3pt,minimum height=0.56cm,fill=blue!4},
    signal/.style={-{Stealth[length=1.5mm]},line width=0.65pt,
        draw=black!80},
    training/.style={-{Stealth[length=1.5mm]},dashed,line width=0.65pt,
        draw=green!35!black},
    loss/.style={block,fill=green!5},
    blocked/.style={dashed,line width=0.65pt,draw=red!65!black}
]
\path[use as bounding box] (0,-0.12) rectangle (8.2,3.88);

\node[block,text width=1.12cm] (input) at (0.75,2.56)
    {Ball evidence\\Context / history};
\node[block,fill=blue!10,text width=1.83cm,minimum height=1.06cm]
    (core) at (3.03,2.56)
    {\textbf{RSSM core $\theta$}\\[2pt]
     Fresh: posterior $q_t$\\Missing: prior $p_t$};
\node[block,text width=1.19cm] (feature) at (5.02,2.56)
    {176D belief\\feature $f_t$};
\node[block,text width=1.21cm] (actor) at (7.04,3.02)
    {Actor $\pi_\phi$\\Walking action};
\node[block,text width=1.21cm] (critic) at (7.04,1.91)
    {Critics $Q_{\psi_i}$};

\draw[signal] (input) -- (core);
\draw[signal] (core) -- (feature);
\draw[signal] (feature.east) -- (actor.west);
\draw[signal] (feature.east) -- (critic.west);

\node[loss,text width=1.18cm] (replay) at (0.75,0.57)
    {Recorded\\replay};
\node[loss,text width=1.83cm] (predictive) at (3.03,0.57)
    {Prediction loss $\mathcal L_M$};
\node[loss,text width=1.25cm] (td) at (6.08,0.57)
    {Critic TD loss\\$\mathcal L_Q$};

\draw[training] (replay.east) -- (predictive.west);
\draw[training] (predictive.north) -- (core.south);
\draw[training] (replay.south) -- (0.75,0.04)
    -- (6.08,0.04) -- (td.south);
\draw[training] (critic.south) -- (7.04,1.20)
    -- (6.08,1.20) -- (td.north);
\draw[training] (td.west) -- (4.70,0.57)
    -- (4.70,1.49) -- (3.77,1.49) -- (3.77,2.03);

% The capped path denotes a prohibited gradient, not a core update.
\draw[blocked] (actor.north) -- (7.04,3.70)
    -- node[above,fill=white,inner sep=1pt,text=red!65!black]
        {Actor gradient to core: stopped}
    (3.03,3.70) -- (3.03,3.29);
\draw[draw=red!65!black,line width=0.9pt]
    (2.92,3.29) -- (3.14,3.29);
\end{tikzpicture}
\caption{Solid arrows show filtering and control; dashed arrows denote replay
supervision. Fresh ball evidence selects the posterior; missing evidence
selects the prior. Prediction and critic TD losses train the core, while
actor gradients stop at the belief feature.}
\label{fig:method_overview}
\end{figure}

